GLM-Dialog: Noise-tolerant Pre-training for Knowledge-grounded Dialogue Generation

We present GLM-Dialog, a large-scale language model (LLM) with 10B parameters capable of knowledge-grounded conversation in Chinese using a search engine to access the Internet knowledge. GLM-Dialog offers a series of applicable techniques for exploiting various external knowledge including both helpful and noisy knowledge, enabling the creation of robust knowledge-grounded dialogue LLMs with limited proper datasets. To evaluate the GLM-Dialog more fairly, we also propose a novel evaluation method to allow humans to converse with multiple deployed bots simultaneously and compare their performance implicitly instead of explicitly rating using multidimensional metrics.Comprehensive evaluations from automatic to human perspective demonstrate the advantages of GLM-Dialog comparing with existing open source Chinese dialogue models. We release both the model checkpoint and source code, and also deploy it as a WeChat application to interact with users. We offer our evaluation platform online in an effort to prompt the development of open source models and reliable dialogue evaluation systems. The additional easy-to-use toolkit that consists of short text entity linking, query generation, and helpful knowledge classification is also released to enable diverse applications. All the source code is available on Github.

==> 5.availability.tex <==
We offer a repository that enables practical usage for Chinese dialogue researchers and developers at \url{https://github.com/RUCKBReasoning/GLM-dialog}. In particular, we 
publish the publicly available resources as well as the reproduction details of our whole system, which includes the contents listed below:

% \textbf{(1) Training Corpus.} We integrate the high-quality datasets as introduced in Section \ref{sec:aproach}. Furthermore, we publish a ~11MB dialogue-format corpus from diverse public Chinese social media Developers and researchers can swiftly conduct dialogue model training upon this corpus.

\textbf{(1) \emph{Model Checkpoint}: We provide all the checkpoints of GLM-dialog publicly as well as the relevant source codes, which may assist the exploration on building personalized, human-like dialogue systems. Meanwhile, we promise that the future versions of GLM-dialog will also be released in this repository.

(2) \emph{Evaluation Platform}: As introduced in Section \ref{sec:evaluation}, we propose an online evaluation platform that can implicitly compare different chatbots. To encourage the development of the community, we also publish the source codes and the access to participate in our evaluation and call for more open-source dialogue services.

(3) \emph{Service and Toolkit}: We build an example dialogue service on WeChat Platform via XDAI framework~\cite{yu2022xdai}, and the same service API is also released publicly. Furthermore, we provide a series of easy-to-use tools for developing chatbots in Chinese, including the entity linking, knowledge classification, web search, etc. 

